A Closer Look at Temporal Ordering in the Segmentation of Instructional Videos

Understanding the steps required to perform a task is an important skill for AI systems. Learning these steps from instructional videos involves two subproblems: (i) identifying the temporal boundary of sequentially occurring segments and (ii) summarizing these steps in natural language. We refer to this task as Procedure Segmentation and Summarization (PSS). In this paper, we take a closer look at PSS and propose three fundamental improvements over current methods. The segmentation task is critical, as generating a correct summary requires each step of the procedure to be correctly identified. However, current segmentation metrics often overestimate the segmentation quality because they do not consider the temporal order of segments. In our first contribution, we propose a new segmentation metric that takes into account the order of segments, giving a more reliable measure of the accuracy of a given predicted segmentation. Current PSS methods are typically trained by proposing segments, matching them with the ground truth and computing a loss. However, much like segmentation metrics, existing matching algorithms do not consider the temporal order of the mapping between candidate segments and the ground truth. In our second contribution, we propose a matching algorithm that constrains the temporal order of segment mapping, and is also differentiable. Lastly, we introduce multi-modal feature training for PSS, which further improves segmentation. We evaluate our approach on two instructional video datasets (YouCook2 and Tasty) and observe an improvement over the state-of-the-art of $\sim7\%$ and $\sim2.5\%$ for procedure segmentation and summarization, respectively.

==> sections/introduction_old.tex <==
Time is a crucial dimension and enables us to learn the evolution of object relationships and states. It is essential for AI system to learn the temporal knowledge in videos to benefit various applications such as video summarization~\cite{Papalampidi_Keller_Lapata_2021,zhang2016video}, describing videos ~\cite{yao2015describing}, story understanding~\cite{han2019contextualized} and timeline construction~\cite{zhou2020temporal}. An essential step to learning such temporal knowledge is identifying events performed by objects and relations among different events over time. Among the different relation types that could exist in the events, we focus on the sequential event order to perform a certain goal-oriented task. Such an encoded temporal event structure can be referred as \textit{procedural knowledge}, and each event is referred as \textit{procedure-segment} or \textit{segment} ~\cite{ZhXuCoCVPR18} to complete a complex procedure e.g. sequential steps to \textit{make onion rings}. These sequential segments follow the arrow of time i.e. each segment follows the next. Apart from inferring segments and understanding scene dynamics, it is necessary for modern AI systems to summarize the segment in a single sentence, as the segment could contain multiple actions or sub-activities ~\cite{ZhXuCoCVPR18}. 
% Different from captioning which usually describe the visual content of an image or video, the current task requires to summarize the procedure segment with a single sentence, as the segment could contain multiple actions or sub-activities ~\cite{ZhXuCoCVPR18}. 

How-to videos on the web (YouTube or Vimeo), such as cooking or repairing household items are a common source to learn diverse knowledge. The instructional videos have a significant property of temporal structure in the segments and these segments are non-overlapping with long term dependencies. Hence, large-scale labeled data ~\cite{Kuehne16end,zhukov2019cross,ZhXuCoCVPR18,tang2019coin} is available to help research towards learning the goal-oriented procedures from instructional videos. This motivates us to identify and summarize the procedure segments in instructional videos, we call this \textit{Dense Procedure Summarization (DPS)}. We refer to the task as \textit{summarization} due to the nature of generating a single sentence for multiple actions in the procedure segment in contrast to captioning, where one needs to generate a sentence to describe the visual content.
% This is different from usual captioning, where the AI system need to describe the content of given visual modality. 
Moreover, the DPS is challenging due to linguistic and visual ambiguity in learning the temporal structure. For example, ingredients mixed with egg and cider is referred to as batter - a linguistic ambiguity due to the referring expression (refer Figure.\ref{fig:overview}).
% Moreover, visual ambiguity arises due to state changes e.g. battered onions changes visual appearance after fried in hot oil.
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{images/overview_2.pdf}
\caption{The pipeline of performing Dense Procedure summarization and Dense Video Captioning~\cite{krishna2017dense}. The pre-extracted features are computed offline. In a single stage, the training pipeline first generates $N$ proposals with a confidence score (between 0 and 1) and then a matching algorithm finds matched pairs between the ground-truth and the generated proposals to compute the loss. Finally, the matched proposals are utilized to summarize the segments and compute language generation loss.  }
\label{fig:overview}
\end{figure*}

% The dense procedure summarization is introduced by Zhou \etal~\cite{ZhXuCoCVPR18} with a YouCook2 dataset, however their work focuses only on procedure segmentation and lacks ~\ls{very strong statement} in procedure summarization. The community has explored the YouCook2 dataset with a closely related task of \textit{Dense Video Captioning} (DVC)~\cite{krishna2017dense}, which focuses on loosely-coupled \ls{not sure what this means} and overlapping events in open domain. \ls{This statement should be stronger, this is one of your core messages} 
Zhou \etal~\cite{ZhXuCoCVPR18} took initial steps to tackle the dense procedure summarization by introducing the YouCook2 dataset, an untrimmed instructional video dataset, and proposing an LSTM-based procedure segmentation method. Subsequently, the researchers ~\cite{zhou2018end, shi2019dense} tackle this problem with a closely related task of \textit{Dense Video Captioning} (DVC)~\cite{krishna2017dense}, which focuses on loosely-coupled and overlapping events in the open domain. However, the inherent property of instructional videos, i.e. procedure segments are non-overlapping and have sequential structure, is ignored. Specifically, the instructional videos focus on a goal, and the main subject performs the steps sequentially, and the steps can not overlap, e.g. one cannot dip onions into the batter without preparing batter (refer Figure.\ref{fig:overview}). Interestingly, we can utilize the existing training pipeline of DVC to perform the current task, i.e. (i) video encoding, (ii) procedure proposal generation and matching, and (iii) matched proposal summary (refer Figure.\ref{fig:overview}). In the current work, we utilize PDVC~\cite{wang2021end} and propose changes in the proposal matching module to exploit the non-overlapping property of procedure segments to improve the performance of DPS. Moreover, the current techniques utilize models pre-trained with a single modality to pre-compute the features; however, the current task (DPS) is multi-modal. Hence, we propose to utilize multi-modal features incorporating visual and textual semantic information into the pipeline without including the video transcript, as instructional videos often lack the transcripts, e.g. videos in the Tasty videos~\cite{sener2019zero}.

The current evaluation framework for DVC systems~\cite{krishna2017dense} and the procedure segmentation metric (mean IoU)~\cite{ZhXuCoCVPR18} are inappropriate for measuring the localization performance of DPS due to their lacking ability to penalize the redundant segments. To appropriately and correctly evaluate sequential procedure segments, we need a framework that can consider the ordering of segments and can penalize redundant segments. In this work, we first analyze the issue in evaluation frameworks and show that the current state-of-the-art methods perform worse than the uniform baselines. Hence, inspired by SODA-C~\cite{fujita2020soda}, an evaluation method to measure the ordered captions score, we propose to use SODA-F1, a dynamic programming-based method that finds the optimal matching between generated and reference procedure segments by considering their temporal orders. Finally, we show that the proposed modifications to PDVC~\cite{wang2021end} achieve state-of-the-art results on YouCook2~\cite{ZhXuCoCVPR18} and the first benchmark on Tasty~\cite{sener2019zero} in the new evaluation framework.

% Procedural learning is beneficial to enable AI systems with an ability to perform goal oriented tasks. 
% \begin{itemize}
%     \item Introduce the concept of procedure learning from instructional videos with comparison to prior work with fixed event space to unconstrained.
%     \item mention the close relation with Dense video captioning~\cite{krishna2017dense} (DVC) and differ by explaining the overlapping/non-overlapping events/steps. Moreover, different from prior prodecure learning dataset, we explore the domain of imperative english sentences to describe the events in contrast to fixed set of labels (e.g. <verb>\_<object>)
%     \item Explaing why we cannot utilize the Dense Video captioning based evaluation metrics -> (i) IOU based metric is biased, (ii) precision/recall detection based are not appropriate as at test time we do not want the different event proposal boundaries, but the optimal segments which can divide the video into non-overlapping event segments. Thus sequential optimal matching must be utilized to evaluate the performance. 
%     \item We build on PDVC~\cite{wang2021end}, a DVC based method and propose to utilize sequential matching based algorithm, SODA~\cite{fujita2020soda}, for evaluation and differentiable version to improve the performance. We also, experiment with multiple video encoding features and identify that multi-modal (video/text) features are more beneficial for the current task.
% \end{itemize}
\paragraph{Contributions}
\begin{itemize}
    \itemsep0em 
    \item We investigate the inefficient current evaluation metrics to measure the procedure segment localization, which fails to consider the sequential order of segments. We propose to utilize the modified SODA-F1~\cite{fujita2020soda}, a dynamic programming-based metric that considers segments' sequential order.
    \item We modify the PDVC~\cite{wang2021end} to incorporate sequential proposal matching to exploit the non-overlapping nature of procedure segments and improve the procedure segment localization performance by a significant margin.
    \item We explore the different video feature representations and demonstrate that multi-modal features are significantly better for the current task.
    \item We demonstrate our approach on two instructional video datasets (YouCook2~\cite{zhou2018end} and Tasty~\cite{sener2019zero}) and achieve new state-of-the-art results on dense procedure summarization.
\end{itemize}
